Powered Dirichlet Process for Controlling the Importance of "Rich-Get-Richer" Prior Assumptions in Bayesian Clustering

One of the most used priors in Bayesian clustering is the Dirichlet prior. It can be expressed as a Chinese Restaurant Process. This process allows nonparametric estimation of the number of clusters when partitioning datasets. Its key feature is the "rich-get-richer" property, which assumes a cluster has an a priori probability to get chosen linearly dependent on population. In this paper, we show that such prior is not always the best choice to model data. We derive the Powered Chinese Restaurant process from a modified version of the Dirichlet-Multinomial distribution to answer this problem. We then develop some of its fundamental properties (expected number of clusters, convergence). Unlike state-of-the-art efforts in this direction, this new formulation allows for direct control of the importance of the "rich-get-richer" prior.

==> biblio_with_doi.tex <==
@article{PastorSatorras2015,
   title={Epidemic processes in complex networks},
   volume={87},
   number={3},
   journal={Reviews of Modern Physics},
   publisher={American Physical Society (APS)},
   author={Pastor-Satorras, Romualdo and Castellano, Claudio and Van Mieghem, Piet and Vespignani, Alessandro},
   year={2015},
   pages={925–979}
}

@article{rodriguez2013modeling,
    title={Modeling Information Propagation with Survival Theory},
    author={Manuel Gomez Rodriguez and Jure Leskovec and Bernhard Schoelkopf},
    year={2013},
    journal={30th International Conference on Machine Learning},
}

@article{DKempeMaxSpreadInfSocNet,
     title={Maximizing the Spread of Influence through a Social Network},
     author={David Kempe and Jon Kleinberg and Eva Tardos},
     journal={Theory of computing},
     volume={11},
     year={2015},
     pages={105-147}
}

@article{pouxmdard2019influential,
    title={Influential spreaders for recurrent epidemics on networks},
    author={Gaël Poux-Médard and Romualdo Pastor-Satorras and Claudio Castellano},
    year={2019},
    journal={Submitted to Phys.Rev.Research},
    eprint={1912.08459},
    archivePrefix={arXiv},
    primaryClass={physics.soc-ph}
}

@article{CoC,
    author = {Myers, Seth and Leskovec, Jure},
    year = {2012},
    pages = {539-548},
    title = {Clash of the Contagions: Cooperation and Competition in Information Diffusion},
}


@article{GTCompetition,
    author = {Mehrdad Agha Mohammad Ali Kermani and Seyed Farshad Fatemi Ardestani  and Alireza Aliahmadi  and Farnaz Barzinpour},
    year = {2017},
    pages = {570-582},
    title = {A novel game theoretic approach for modeling competitive information diffusion in social networks with heterogeneous nodes},
    volume={466},
    journal={Physica A},
}

@article{GTCompetition2,
    author = {Wu, Hong and Liu, Weiyi and Yue, Kun and Huang, Weipeng and Yang, Ke},
    year = {2015},
    pages = {516-519},
    title = {Maximizing the Spread of Competitive Influence in a Social Network Oriented to Viral Marketing},
}


@article{GTCompetition3,
    author = {Bharathi, Shishir and Kempe, David and Salek, Mahyar},
    title = {Competitive Influence Maximization in Social Networks},
    year = {2007},
    publisher = {Springer-Verlag},
    address = {Berlin, Heidelberg},
    booktitle = {3rd International Conference on Internet and Network Economics},
    pages = {306–311},
    numpages = {6},
    series = {WINE’07}
}


@article{SpreadNewsOnlineScience,
    author = {Soroush Vosoughi and Deb Roy and Sinon Aral},
    year = {2018},
    pages = {1146-1151},
    title = {The spread of true and false news online},
    journal={Science},
}

@article{SpreadNewsOnlineWWW,
    author = {Romero, Daniel and Meeder, Brendan and Kleinberg, Jon},
    year = {2011},
    pages = {695-704},
    title = {Differences in the Mechanics of Information Diffusion Across Topics: Idioms, Political Hashtags, and Complex Contagion on Twitter},
    volume = {695-704},
    journal = {WWW},
}


@article{InteractingViruses,
    author = {Beutel, Alex and Prakash, B. and Rosenfeld, Roni and Faloutsos, Christos},
    year = {2012},
    title = {Interacting viruses in networks: Can both survive?},
    journal = {Proceedings of the ACM SIGKDD},
}

@article{ReviewSBM,
   title={Stochastic block models: A comparison of variants and inference methods},
   author={Thorben Funke and Till Becker},
   journal={PloS one},
   year={2019},
}

@article {AntoniaScalableRS,
	author = {Godoy-Lorite, Antonia and Guimer{\`a}, Roger and Moore, Cristopher and Sales-Pardo, Marta},
	title = {Accurate and scalable social recommendation using mixed-membership stochastic block models},
	volume = {113},
	number = {50},
	pages = {14207--14212},
	year = {2016},
	publisher = {National Academy of Sciences},
	journal = {PNAS}
}


@article{SymptDiseNet,
    author = {Zhou, Xuezhong and Menche, Jörg and Barabasi, Albert-Laszlo and Sharma, Amitabh},
    year = {2014},
    pages = {4212},
    title = {Human symptoms–disease network},
    volume = {5},
    journal = {Nature communications},
}

@article{AiroldiMMSBM,
    author = {Airoldi, Edoardo and Blei, D.M. and Fienberg, S.E. and Xing, E.P.},
    year = {2008},
    pages = {1991-1992},
    title = {Mixed Membership Stochastic Blockmodels},
    volume = {9},
    journal = {Journal of Machine Learning Research}
}

@article{Calibration,
    author = {Gneiting, T. and Raftery, A. and Balabdaoui, F. and Westveld, Anton},
    year = {2003},
    title = {Verifying probabilistic forecasts: Calibration and sharpness}
}

@article{MFReco,
    author={Y. {Koren} and R. {Bell} and C. {Volinsky}},
    journal={Computer},
    title={Matrix Factorization Techniques for Recommender Systems},
    year={2009},
    volume={42},
    number={8},
    pages={30-37},
}

@article{SEESdrugdrugInter,
    author={Roger Guimerà and Marta Sales-Pardo},
    journal={PLoS Comput Biol},
    title={A Network Inference Method for Large-Scale Unsupervised Identification of Novel Drug-Drug Interactions},
    year={2013},
}

@article{wang2012scalable,
  title={Scalable influence maximization for independent cascade model in large-scale social networks},
  author={Wang, Chi and Chen, Wei and Wang, Yajun},
  journal={Data Mining and Knowledge Discovery},
  volume={25},
  number={3},
  pages={545-576},
  year={2012},
  publisher={Springer}
}


@article{CombinLanguage,
    author = {Loreto, Vittorio and Gravino, Pietro and Servedio, Vito D. P. and Tria, Francesca},
    title = {On the Emergence of Syntactic Structures: Quantifying and Modeling Duality of Patterning},
    journal = {Topics in Cognitive Science},
    volume = {8},
    number = {2},
    pages = {469-480},
    year = {2016}
}

@article{OpinionsCoevol,
    author = {Nigam, Aastha and Shin, Kijung and Bahulkar, Ashwin and Hooi, Bryan and Hachen, David and Szymanski, Boleslaw and Faloutsos, Christos and Chawla, Nitesh},
    year = {2019},
    pages = {122-140},
    title = {ONE-M: Modeling the Co-evolution of Opinions and Network Connections, ECML PKDD, 10–14, 2018, Part II},
}

@article{DataSetTwitter,
    author = {Nathan O. Hodas and Kristina Lerman},
    year = {2014},
    journal={Scientific Reports},
    volume={4},
    number={4343},
    title = {The Simple Rules of Social Contagion},
}

@inbook{Bishop,
    author = {Bishop, Christopher},
    year = {2006},
    month = {01},
    pages = {450-455},
    title = {Pattern Recognition and Machine Learning},
    volume = {16},
    journal = {Journal of Electronic Imaging},
    %doi = {10.1117/1.2819119}
}


@article{Yuchung1987,
    author = {Yuchung J. Wang  and  George Y. Wong },
    title = {Stochastic Blockmodels for Directed Graphs},
    journal = {Journal of the American Statistical Association},
    volume = {82},
    number = {397},
    pages = {8-19},
    year  = {1987},
    publisher = {Taylor & Francis},
    %doi = {10.1080/01621459.1987.10478385},
}

@article{refChoixAIC,
    author = {A. Salah and M. Nadif},
    title = {Directional co-clustering},
    journal = {Adv. Data Anal. Classical},
    volume = {3},
    number = {13},
    pages = {591-620},
    year  = {2019},
}

@article{Akaike1973,
    author = {H. Akaike},
    title = {Information Theory and an Extension of the Maximum Likelihood Principle},
    journal = {2nd International Symposium on Information Theory},
    pages = {267-281},
    year  = {1973},
}

@article{InfoPath,
    title={Structure and Dynamics of Information Pathways in Online Media},
    author={Manuel Gomez Rodriguez and Jure Leskovec and Bernhard Schoelkopf},
    year={2013},
    journal={WSDM},
}


@inproceedings{kong2019,
    author = {Kong, Quyu and Rizoiu, Marian-Andrei and Xie, Lexing},
    year = {2020},
    month = {01},
    pages = {286-294},
    booktitle = {Proceedings of the 13th International Conference on Web Search and Data Mining},
    title = {Modeling Information Cascades with Self-exciting Processes via Generalized Epidemic Models},
    %doi = {10.1145/3336191.3371821},
    series = {WSDM ’20}
}

@inproceedings{sun2020,
    author = {Sun, Lichao and Chen, Albert and Yu, Philip S. and Chen, Wei},
    title = {Influence Maximization with Spontaneous User Adoption},
    year = {2020},
    publisher = {Association for Computing Machinery},
    %doi = {10.1145/3336191.3371791},
    booktitle = {Proceedings of the 13th International Conference on Web Search and Data Mining},
    pages = {573–581},
    numpages = {9},
    series = {WSDM ’20}
}

@article{SergioSocialDilemma,
author = {Cobo-López, S., Godoy-Lorite, A., Duch, J. et al. },
year = {2018},
title = {Optimal prediction of decisions and model selection in social dilemmas using block models},
volume = {7(48)},
journal = {EPJ Data Sci},
%doi = {10.1140/epjds/s13688-018-0175-3}
}

@Article{MrBanks,
author = {Mario Gutiérres-Roig and Carlota Segura and Jordi Dutch and Josep Perello},
title = {Market Imitation and Win-Stay Lose-Shift Strategies Emerge as Unintended Patterns in Market Direction Guesses},
journal={PLOS One},
year = {2016},
}

@Article{HumanPrefSBM,
author = {Roger Guimera and Alejandro Llorente and Marta Sales-Pardo},
title = {Predicting Human Preferences Using the Block Structure of Complex Social Networks},
journal={PLOS One},
year = {2012},
volume={7},
number={9}
}

@article{IMMSBM,
    title={Interactions in information spread: quantification and interpretation using stochastic block models},
    author={Gaël Poux-Médard and Julien Velcin and Sabine Loudcher},
    year={2020},
    eprint={2004.04552},
    journal={arXiv},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@article{Chunyuan2019,
    title={Adversarial Learning of a Sampler Based on an Unnormalized Distribution},
    author={Chunyuan Li, Ke Bai, Jianqiao Li, Guoyin Wang, Changyou Chen, Lawrence Carin},
    year={2019},
    journal={Proceedings of Machine Learning Research},
    archivePrefix={PMLR},
}

@article{Gutmann2013,
author = {Gutmann, M., Hyvärinen, A.},
title = {Estimation of unnormalized statistical models without numerical integration},
journal={Proceedings of the Sixth Workshop on Information Theoretic Methods in Science and Engineering (WITMSE)},
year = {2013},
volume={6},
}

@article{Sethuraman1994,
author = {Sethuraman J.},
title = {A constructive definition of Dirichlet priors},
journal={Statistica sinica},
year = {1994},
volume={4},
number={4},
pages={639-650}
}

@article{Wilks1992,
author = {Wilks, S.S.},
title = {Mathematical statistics},
publisher={John Wiley},
year = {1992},
pages={section 7},
}

@inproceedings{wallach2010,
  title={An alternative prior process for nonparametric Bayesian clustering},
  author={Wallach, Hanna and Jensen, Shane and Dicker, Lee and Heller, Katherine},
  booktitle={Proceedings of the Thirteenth International Conference on Artificial Intelligence and Statistics},
  pages={892-899},
  year={2010},
  organization={JMLR}
}

@inproceedings{Jensen2008,
  title={Bayesian clustering of transcription factor binding motifs},
  author={Jensen, S. and Liu, J.},
  booktitle={Journal of the American Statistical Association},
  pages={188–200},
  year={2008},
  volume={103},
}

@inproceedings{Qin2003,
  title={Identification of co-regulated genes through Bayesian clustering of predicted regulatory binding sites},
  author={Qin, Z. S. and McCue, L. A. and Thompson, W. and Mayerhofer, L. and Lawrence, C. E. and Liu, J. S.},
  booktitle={Nature Biotechnology},
  pages={435–439},
  year={2003},
  volume={21},
}

@inproceedings{Driver1932,
  author={Driver H.E. and Kroeber A.L.},
  booktitle={Quantitative expression of cultural relationships},
  publisher={University of California Press},
  year={1932},
}

@article{mcdowell2018,
  title={Clustering gene expression time series data using an infinite Gaussian process mixture model},
  author={McDowell, Ian C and Manandhar, Dinesh and Vockley, Christopher M and Schmid, Amy K and Reddy, Timothy E and Engelhardt, Barbara E},
  journal={PLoS computational biology},
  volume={14},
  number={1},
  pages={e1005896},
  year={2018},
  publisher={Public Library of Science}
}

@article{Jelodar2017,
author = {Jelodar, Hamed and Wang, Yongli and Yuan, Chi and Feng, Xia},
year = {2017},
month = {11},
pages = {},
title = {Latent Dirichlet Allocation (LDA) and Topic modeling: models, applications, a survey}
}

@article{LDA2003,
author = {Blei, David M. and Ng, Andrew Y. and Jordan, Michael I.},
title = {Latent Dirichlet Allocation},
year = {2003},
issue_date = {3/1/2003},
publisher = {JMLR.org},
volume = {3},
issn = {1532-4435},
journal = {J. Mach. Learn. Res.},
pages = {993–1022},
numpages = {30}
}

@article{Ferguson1973,
author = {Thomas S. Ferguson},
title = {{A Bayesian Analysis of Some Nonparametric Problems}},
volume = {1},
journal = {The Annals of Statistics},
number = {2},
publisher = {Institute of Mathematical Statistics},
pages = {209 -- 230},
year = {1973},
%doi = {10.1214/aos/1176342360},
}

@article{PitmanYor1997,
author = {Jim Pitman and Marc Yor},
title = {{The two-parameter Poisson-Dirichlet distribution derived from a stable subordinator}},
volume = {25},
journal = {The Annals of Probability},
number = {2},
publisher = {Institute of Mathematical Statistics},
pages = {855 -- 900},
keywords = {Local time, Poisson point process, ranked lengths of excursions, semistable Markov process, Zero set},
year = {1997},
%doi = {10.1214/aop/1024404422},
}

@article{Ishwaran2003,
author = {Ishwaran, Hemant and James, Lancelot},
year = {2003},
month = {10},
pages = {1211-1235},
title = {Generalized weighted Chinese restaurant processes for species sampling mixture models},
volume = {13},
journal = {Statistica Sinica}
}

@inproceedings{Sudderth2009,
 author = {Sudderth, Erik and Jordan, Michael},
 booktitle = {NIPS},
 title = {Shared Segmentation of Natural Scenes Using Dependent Pitman-Yor Processes},
 volume = {21},
 year = {2009}
}

@article{Goldwater2011,
  author  = {Sharon Goldwater and Thomas L. Griffiths and Mark Johnson},
  title   = {Producing Power-Law Distributions and Damping Word Frequencies with Two-Stage Language Models},
  journal = {JMLR},
  year    = {2011},
  volume  = {12},
  number  = {68},
}


@article{Arratia1992,
 ISSN = {10505164},
 author = {Richard Arratia and A. D. Barbour and Simon Tavaré},
 journal = {The Annals of Applied Probability},
 number = {3},
 pages = {519--535},
 publisher = {Institute of Mathematical Statistics},
 title = {Poisson Process Approximations for the Ewens Sampling Formula},
 volume = {2},
 year = {1992}
}

@inproceedings{Rasmussen1999,
author = {Rasmussen, Carl Edward},
title = {The Infinite Gaussian Mixture Model},
year = {1999},
publisher = {MIT Press},
pages = {554–560},
numpages = {7},
location = {Denver, CO},
series = {NIPS'99}
}

@inproceedings{Kamper2014,
  title={Gibbs sampling for fitting finite and infinite Gaussian mixture models},
  author={H. Kamper},
  year={2014}
}

@inproceedings{Yin2014,
author = {Yin, Jianhua and Wang, Jianyong},
title = {A Dirichlet Multinomial Mixture Model-Based Approach for Short Text Clustering},
year = {2014},
isbn = {9781450329569},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
%doi = {10.1145/2623330.2623715},
booktitle = {Proceedings of the 20th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
pages = {233–242},
numpages = {10},
keywords = {short text clustering, dirichlet multinomial mixture, gibbs sampling},
location = {New York, New York, USA},
series = {KDD '14}
}

@article{Hanson2017,
author = {Hanson, J. W.  and Ortman, S. G.  and Lobo, J. },
title = {Urbanism and the division of labour in the Roman Empire},
journal = {Journal of The Royal Society Interface},
volume = {14},
number = {136},
pages = {20170367},
year = {2017},
%doi = {10.1098/rsif.2017.0367},
}

@book{Hanson2016,
  title={An urban geography of the Roman world, 100 BC to AD 300},
  author={Hanson, John William},
  volume={18},
  year={2016},
  publisher={Archaeopress Oxford}
}

@inproceedings{Ghosh2014,
author = {Ghosh, Soumya and Raptis, Michalis and Sigal, Leonid and Sudderth, Erik B.},
title = {Nonparametric Clustering with Distance Dependent Hierarchies},
year = {2014},
pages = {260–269},
numpages = {10},
series = {UAI'14}
}

@article{Socher2011,
author = {Socher, Richard and Maas, Andrew and Manning, Christopher},
year = {2011},
pages = {698-706},
title = {Spectral Chinese Restaurant Processes: Nonparametric Clustering Based on Similarities},
volume = {15},
journal = {JMLR - Proceedings}
}


@article{Blei2011,
author = {Blei, D.M. and Frazier, Peter},
year = {2011},
month = {08},
pages = {2461-2488},
title = {Distance dependent Chinese restaurant processes},
volume = {12},
journal = {Journal of Machine Learning Research}
}

@inproceedings{welling2006,
  title={Flexible priors for infinite mixture models},
  author={Welling, Max},
  booktitle={Workshop on learning with non-parametric Bayesian methods},
  year={2006},
}

@article{Ghitza2013,
    author = {Ghitza, Yair and Gelman, Andrew},
    year = {2013},
    month = {07},
    pages = {},
    title = {Deep Interactions with MRP: Election Turnout and Voting Patterns Among Small Electoral Subgroups},
    volume = {57},
    journal = {American Journal of Political Science},
    doi = {10.1111/ajps.12004}
}

@article{McCarthy2012DifferentialEA,
  title={Differential expression analysis of multifactor RNA-Seq experiments with respect to biological variation},
  author={Davis J. McCarthy and Y. Chen and G. Smyth},
  journal={Nucleic Acids Research},
  year={2012},
  volume={40},
  pages={4288 - 4297}
}

@article{Khurshid2005ConfidenceIntervNegBinDist,
author = {Khurshid, Anwer and Ageel, Mohammad and Lodhi, Rizwan},
year = {2005},
month = {01},
pages = {59-70},
title = {On Confidence Intervals for the Negative Binomial Distribution},
volume = {26},
journal = {Revista Investigacion Operacional}
}


